CLASP: Few-Shot Cross-Lingual Data Augmentation for Semantic Parsing

A bottleneck to developing Semantic Parsing (SP) models is the need for a large volume of human-labeled training data. Given the complexity and cost of human annotation for SP, labeled data is often scarce, particularly in multilingual settings. Large Language Models (LLMs) excel at SP given only a few examples, however LLMs are unsuitable for runtime systems which require low latency. In this work, we propose CLASP, a simple method to improve low-resource SP for moderate-sized models: we generate synthetic data from AlexaTM 20B to augment the training set for a model 40x smaller (500M parameters). We evaluate on two datasets in low-resource settings: English PIZZA, containing either 348 or 16 real examples, and mTOP cross-lingual zero-shot, where training data is available only in English, and the model must generalize to four new languages. On both datasets, we show significant improvements over strong baseline methods.

==> ablations.tex <==

Our baseline model (``dev-only'') is trained only on the 348 utterances from the development set.
In all other methods where we add more data, we up-sample the dev set so it always accounts for 50\% of the instances seen during training.

We explore adding samples from the provided training set (``train''), 
in increments of 1x, 2x, 5x, and 10x
of 348 samples.
(We choose 348 since it is the same size as the dev set.)

For generation, we consider three scenarios,
all following the method described in section \ref{sec:method_mono},
with slight variations:
(1) ``train-regen'': use the in-context prompts to re-generate the text from the parse;
(2) ``dev-para'': use the in-context prompts for parse-to-text from the dev set, but do \textit{not} change the slots;
(3) ``dev-slot-repl'': As described in section \ref{sec:method_mono},
replace one slot with a different value from the catalog, and generate a corresponding natural language text.

We explore ``tagging'' the synthetic data with \texttt{<synthetic>}, inspired by
Tagged Back-Translation (\citealt{caswell-etal-2019-tagged,marie-etal-2020-tagged}).




\subsubsection{mTOP Experiment Runs}

As an upper bound, we train on all languages jointly, achieving X.
Then, as a starting point, we follow the standard zero-shot setup, training only on English data,
then testing on all languages.

Our baseline method uses the 20B model to translate the text, then we use
Sim-Align \cite{jalili-sabet-etal-2020-simalign} to align the translated text back to the slot labels,
to be able to recover the target parse.
We use 'xlm-roberta-base' as the alignment model, with ArgMax alignment strategy.
We also tried IterMax and the final results were nearly identical.
See details in the Appendix.

Finally, as described in section \ref{sec:method_cross}, for our candidate model
we first translate the slots with 20B,
then use a one-shot in-context prompt to generate the parse.
We filter the outputs as shown in Appendix TODO.

We assume that the target intent distribution for each language is known,
and is fixed to be the distribution in the full dataset.
In cases where we discard generated utterances,
we duplicate the English sentence corresponding to that utterance
(utilizing the fact that mTOP is parallel with utterance IDs)
to maintain the target class distribution.
